Performance of the image persistence model for Euclid infrared detectors

Large-format infrared detectors are at the heart of major ground and space-based astronomical instruments, and the HgCdTe HxRG is the most widely used. The Near Infrared Spectrometer and Photometer (NISP) of the ESA's Euclid mission launched in July 2023 hosts 16 H2RG detectors in the focal plane. Their performance relies heavily on the effect of image persistence, which results in residual images that can remain in the detector for a long time contaminating any subsequent observations. Deriving a precise model of image persistence is challenging due to the sensitivity of this effect to observation history going back hours or even days. Nevertheless, persistence removal is a critical part of image processing because it limits the accuracy of the derived cosmological parameters. We will present the empirical model of image persistence derived from ground characterization data, adapted to the Euclid observation sequence and compared with the data obtained during the in-orbit calibrations of the satellite.

==> acronym.tex <==
\acrodef{ADU}{Analog Digital Unit}
\acrodef{ADS}{Airbus Defence \& Space}
\acrodef{ASIC}{application specific integrated circuit}
\acrodef{BFE}{brighter-fatter effect}
\acrodef{CaLA}{camera-lens assembly}
\acrodef{CCD}{charge-coupled device}
\acrodef{CoLA}{corrector-lens assembly}
\acrodef{CDS}{Correlated Double Sampling}
\acrodef{CFC}{cryo-flex cable}
\acrodef{CGH}{computer-generated hologram}
\acrodef{CNES}{Centre National d'Etude Spacial}
\acrodef{CPPM}{Centre de Physique des Particules de Marseille}
\acrodef{CPU}{central processing unit}
\acrodef{CTE}{coefficient of thermal expansion}
\acrodef{DE}{Dark Energy}
\acrodef{DM}{Dark Matter}
\acrodef{DCU}{Detector Control Unit}
\acrodef{DPU}{Data Processing Unit}
\acrodef{DS}{Detector System}
\acrodef{EDS}{\Euclid Deep Survey}
\acrodef{EE}{encircled energy}
\acrodef{ESA}{European Space Agency}
\acrodef{EWS}{\Euclid Wide Survey}
\acrodef{FDIR}{Fault Detection, Isolation and Recovery}
\acrodef{FOM}{figure of merit}
\acrodef{FoV}{field of view}
\acrodef{FPA}{Focal Plane Array}
\acrodef{FWA}{Filter Wheel Assembly}
\acrodef{FWC}{full-well capacity}
\acrodef{FWHM}{full width at half maximum}
\acrodef{GWA}{Grism Wheel Assembly}
\acrodef{H2RG}{HAWAII-2RG}
\acrodef{IP2I}{Institut de Physique des 2 Infinis de Lyon}
\acrodef{JWST}{{\em James Webb} Space Telescope}
\acrodef{IAD}{ion-assisted deposition}
\acrodef{ICU}{Instrument Control Unit}
\acrodef{IPC}{inter-pixel capacitance}
\acrodef{L2}{second Lagrange Point}
\acrodef{LAM}{Laboratoire d'Astrophysique de Marseille}
\acrodef{LED}{light-emitting diode}
\acrodef{MACC}{Multiple Accumulated}
\acrodef{MLI}{multi-layer insulation}
\acrodef{MMU}{Mass Memory Unit}
\acrodef{MPE}{Max-Planck-Institut für extraterrestrische Physik}
\acrodef{MPIA}{Max-Planck-Institut für Astronomie}
\acrodef{NA}{numerical aperture}
\acrodef{NASA}{National Aeronautic and Space Administration}
\acrodef{JPL}{NASA Jet Propulsion Laboratory}
\acrodef{MZ-CGH}{multi-zonal computer-generated hologram}
\acrodef{NI-DS}{NISP Detector System}
\acrodef{NI-CU}{NISP Calibration Unit}
\acrodef{NI-ICU}{NISP Instrument Control Unit}
\acrodef{NI-DPU}{NISP Data Processing Unit}
\acrodef{NI-OA}{NISP Optical Assembly}
\acrodef{NI-SA-ST}{Mechanical Support Structure}
\acrodef{NI-SA-HP}{Mechanical Support Hexa Pod}
\acrodef{NI-GWA}{NISP Grism Wheel Assembly}
\acrodef{NI-FWA}{NISP Filter Wheel Assembly}
\acrodef{NI-FPA}{NISP Focal Plane Assembly}
\acrodef{NI-WE}{NISP Warm Electronics}
\acrodef{NISP}{Near-Infrared Spectrometer and Photometer}
\acrodef{PARMS}{plasma-assisted reactive magnetron sputtering}
\acrodef{PLM}{payload module}
\acrodef{PTFE}{polytetrafluoroethylene}
\acrodef{PV}{performance verification}
\acrodef{PWM}{pulse-width modulation}
\acrodef{PSF}{point spread function}
\acrodef{QE}{quantum efficiency}
\acrodef{ROIC}{readout-integrated chip}
\acrodef{ROS}{reference observing sequence}
\acrodef{SCA}{sensor chip array}
\acrodef{SCE}{sensor chip electronic}
\acrodef{SCS}{sensor chip system}
\acrodef{SGS}{Science Ground Segment}
\acrodef{SHS}{Shack-Hartmann sensor}
\acrodef{SNR}[SNR]{signal-to-noise ratio}
\acrodef{SED}{spectral energy distribution}
\acrodef{SiC}{silicon carbide}
\acrodef{SVM}{service module}
\acrodef{VIS}{Visible imaging}
\acrodef{WD}{white dwarf}
\acrodef{WFE}{wavefront error}
\acrodef{ZP}{zero point}

